VideoCrafter1: Open Diffusion Models for High-Quality Video Generation

Video generation has increasingly gained interest in both academia and industry. Although commercial tools can generate plausible videos, there is a limited number of open-source models available for researchers and engineers. In this work, we introduce two diffusion models for high-quality video generation, namely text-to-video (T2V) and image-to-video (I2V) models. T2V models synthesize a video based on a given text input, while I2V models incorporate an additional image input. Our proposed T2V model can generate realistic and cinematic-quality videos with a resolution of $1024 \times 576$, outperforming other open-source T2V models in terms of quality. The I2V model is designed to produce videos that strictly adhere to the content of the provided reference image, preserving its content, structure, and style. This model is the first open-source I2V foundation model capable of transforming a given image into a video clip while maintaining content preservation constraints. We believe that these open-source video generation models will contribute significantly to the technological advancements within the community.

==> fig_tex/eval_videocrafter.tex <==


\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
{VideoCrafter} & Visual & Text-Video & Motion & Temporal \\ 
{Ver. \& Resolution} & Quality & Alignment & Quality & Consistency \\ \midrule

% \multicolumn{6}{c}{User Study}    \\ 
23.04~(256$\times$256)   & 46.88   & 41.56   & \textbf{56.24*}  & 55.78    \\ 
23.09~(1024$\times$576)  & 59.53   & 51.29   & 51.97  & 56.36   \\ 
23.11~(1024$\times$576)  & \textbf{61.64}   &  \textbf{66.76}   & 56.06     &  \textbf{60.36}   \\ 
\bottomrule
\end{tabular}
}
\vspace{-1em}
\caption{
The performance progress on the VideoCrafter model using EvalCrafter~\cite{liu2023evalcrafter}. * for motion quality, the resolution will hugely influence the results.
}
\vspace{-1em}
\label{tab:version}
\end{table}


==> fig_tex/fig_demo3.tex <==
\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.85\linewidth]{figs/demo5.pdf}
   \caption{Visual comparison with Gen-2, Pika Labs, I2VGen-XL, and Zeroscope-XL}
   \label{fig:demo3}
\end{figure*}

==> fig_tex/fig_teaser.tex <==
\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.95\linewidth]{figs/teaser.pdf}
   \caption{We have open-sourced two diffusion models for video generation in VideoCrafter1. The Text-to-Video (T2V) model takes a text prompt as input and generates a video accordingly. On the other hand, the Image-to-Video (I2V) model accepts either an image, a text prompt, or both as input for video generation. }
   \label{fig:framework-t2v}
\end{figure*}
